RELIC: Evaluating Complex Reasoning via the Recognition of Languages In-Context

Large language models (LLMs) are increasingly used to solve complex tasks where they must retrieve and compose many pieces of in-context information in long reasoning chains. For many real-world tasks it is hard to accurately gauge how model performance and strategy change as task complexity grows. To evaluate models' complex reasoning capability in a scalable and verifiable way, we introduce RELIC (Recognition of Languages In-Context), a framework that evaluates an LLM's ability to decide whether a given string belongs to the context-free language (CFL) generated by a grammar presented in-context. CFL recognition allows us to modulate the intrinsic complexity of the problem by varying grammar size and string length and translate this asymptotic complexity into predictions for ideal LLM performance. We find that even the most advanced reasoning models perform poorly on RELIC, not only failing to appropriately scale their inference compute to keep pace with task difficulty, but even reducing the number of reasoning tokens they use as task complexity increases. We find that these decreases in compute accompany changes in reasoning strategy, as models move from identifying and implementing algorithmic solutions to guessing. For models whose full completions go uninspected, this manifests as ``quiet quitting'' on hard tasks.

==> preamble.tex <==
%% Custom packages
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{booktabs}
\usepackage{cleveref}
\usepackage{mathtools}
\usepackage{multirow}
\usepackage{paralist}
\usepackage{physics}
\usepackage{siunitx}
\usepackage{tabularx}
\usepackage{tcolorbox}
\usepackage{textcomp}
\usepackage{wrapfig} 
\usepackage{xcolor}
\makeatletter
% ACL only loads lineno in review mode, but the prompt/LLM boxes use
% internal line numbering in every mode.
\@ifpackageloaded{lineno}{}{\RequirePackage[mathlines]{lineno}}
\makeatother

\newtheorem{lemma}{Lemma}[section]
\newtheorem*{remark}{Remark}
\renewcommand{\qedsymbol}{$\blacksquare$}

\crefformat{section}{\S#2#1#3}
\crefmultiformat{section}{\S\S#2#1#3}{ and~#2#1#3}{, #2#1#3}{, and~#2#1#3}

\sisetup{
  separate-uncertainty = true,
  table-align-uncertainty = true,
  % table-number-alignment = center,
  % round-mode             = places,
  % round-precision        = 2
  % output-open-uncertainty = (,
  % output-open-uncertainty  = {\tiny\,$\pm$\,},
  % output-close-uncertainty = {},
}

\def\affil#1{\textsuperscript{#1}}
\def\CDS{\affil{$\delta$}}
\def\LING{\affil{$\lambda$}}

\definecolor{canvas}{HTML}{fbf8f4}
\definecolor{goldenrod}{HTML}{fdedd7}
\definecolor{persimmon}{HTML}{d65f3d}
\definecolor{mygreen}{RGB}{0,128,0} % A nice shade of green
\definecolor{myred}{RGB}{204,0,0}   % A good shade of red


\newcounter{paranum}
\newcounter{boxpara}
\newbool{tcb@numberparas}
\boolfalse{tcb@numberparas}

\tcbuselibrary{most}
\usetikzlibrary{decorations.pathmorphing}


\makeatletter
\newdimen\chat@zig@amp
\newdimen\chat@zig@seg
\newdimen\chat@zig@x
\newdimen\chat@zig@remaining
\newdimen\chat@zig@step
\newdimen\chat@zig@half
\newdimen\chat@xa
\newdimen\chat@xb
\newdimen\chat@ya
\newcount\chat@zig@count
\newbox\chattitleboxsaved
\chat@zig@amp=0.9mm
\chat@zig@seg=1.4mm

\newcommand{\chattitlebox}{\copy\tcb@titlebox}

\newcommand{\chatzigzagline}[2]{%
  \pgfextractx{\chat@xa}{#1}%
  \pgfextractx{\chat@xb}{#2}%
  \pgfextracty{\chat@ya}{#1}%
  \chat@zig@x=\chat@xa%
  \chat@zig@remaining=\chat@xb%
  \advance\chat@zig@remaining by -\chat@xa%
  \pgfmathsetmacro{\chat@zig@width}{abs((\chat@zig@remaining)/1pt)}%
  \pgfmathsetmacro{\chat@zig@segpt}{\chat@zig@seg/1pt}%
  \pgfmathtruncatemacro{\chat@zig@n}{max(1,round(\chat@zig@width/\chat@zig@segpt))}%
  \chat@zig@count=\chat@zig@n\relax%
  \chat@zig@step=\chat@zig@remaining%
  \ifnum\chat@zig@count>0\relax%
    \divide\chat@zig@step by \chat@zig@count%
  \fi%
  \chat@zig@half=\chat@zig@step%
  \divide\chat@zig@half by 2%
  \pgfpathlineto{\pgfqpoint{\chat@zig@x}{\chat@ya}}%
  \chat@zig@count=0%
  \loop%
    \ifnum\chat@zig@count<\chat@zig@n\relax%
      \advance\chat@zig@x by \chat@zig@half%
      \advance\chat@zig@count by 1%
      \ifodd\chat@zig@count%
        \pgfpathlineto{\pgfqpoint{\chat@zig@x}{\dimexpr\chat@ya+\chat@zig@amp\relax}}%
      \else%
        \pgfpathlineto{\pgfqpoint{\chat@zig@x}{\dimexpr\chat@ya-\chat@zig@amp\relax}}%
      \fi%
      \advance\chat@zig@x by \chat@zig@half%
      \pgfpathlineto{\pgfqpoint{\chat@zig@x}{\chat@ya}}%
  \repeat%
}
\makeatother

\newcommand{\boxpara}{%
  \refstepcounter{boxpara}%
  \hfill{\color{black!50} \texttt{\textpilcrow\arabic{boxpara}}}%
}

% Global paragraph hook: only does something if the boolean is true
\AddToHook{para/begin}{%
  \ifbool{tcb@numberparas}{%
    \stepcounter{boxpara}%
    \vadjust{%
      \smash{%
        \makebox[\linewidth][r]{%
          \scriptsize\color{persimmon}%
          \textpilcrow~\arabic{boxpara}\hspace{0.4em}%
        }%
      }%
    }%
  }{}%
}

\tcbset{
  chatbox/.style={
    enhanced,
    boxrule=0.9pt,
    arc=2pt,
    colback=white,
    left=3mm,right=3mm,top=4mm,bottom=3mm,
    before skip=10pt,
    after skip=10pt,
    breakable = true,
    frame hidden,
    interior hidden,
    underlay boxed title={%
      \global\setbox\chattitleboxsaved=\copy\csname tcb@titlebox\endcsname%
      \global\setbox\csname tcb@titlebox\endcsname=\hbox{}%
    },
    boxed title style={
      arc=5pt,
      boxrule=0.9pt,
      left=1.3mm,
      right=1.3mm,
      top=0.6mm,
      bottom=0.6mm,
    },
    overlay unbroken={},
    overlay first={},
    overlay unbroken app={%
      \pgftext[at={\pgfpointanchor{title}{center}}]{\box\chattitleboxsaved}%
    },
    overlay first app={%
      \pgftext[at={\pgfpointanchor{title}{center}}]{\box\chattitleboxsaved}%
    },
    overlay middle={},
    overlay last={},
    fontupper=\rmfamily\small,
    fonttitle=\scriptsize\sffamily\bfseries,
    attach boxed title to top left={yshift=-3mm,xshift=4mm},
    finish={},
    no underlay unbroken,
    no underlay first,
    no underlay middle,
    no underlay last,
    underlay unbroken={%
      \begin{pgfscope}%
      \pgfsetcornersarced{\pgfqpoint{2pt}{2pt}}%
      \pgfpathmoveto{\pgfpointlineattime{0.02}{\pgfpointanchor{frame}{north west}}{\pgfpointanchor{frame}{south west}}}%
      \pgfpathlineto{\pgfpointanchor{frame}{north west}}%
      \pgfpathlineto{\pgfpointanchor{frame}{north east}}%
      \pgfpathlineto{\pgfpointanchor{frame}{south east}}%
      \pgfpathlineto{\pgfpointanchor{frame}{south west}}%
      \pgfpathclose%
      \pgfsetfillcolor{tcbcolback}%
      \pgfsetfillopacity{1}%
      \pgfsetstrokecolor{tcbcolframe}%
      \pgfsetstrokeopacity{1}%
      \pgfsetlinewidth{0.9pt}%
      \pgfusepath{fill,stroke}%
      \end{pgfscope}%
    },
    underlay first={%
      \begin{pgfscope}%
      \pgfsetcornersarced{\pgfqpoint{2pt}{2pt}}%
      \pgfpathmoveto{\pgfpointlineattime{0.02}{\pgfpointanchor{frame}{north west}}{\pgfpointanchor{frame}{south west}}}%
      \pgfpathlineto{\pgfpointanchor{frame}{north west}}%
      \pgfpathlineto{\pgfpointanchor{frame}{north east}}%
      \pgfpathlineto{\pgfpointanchor{frame}{south east}}%
      \pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
      \chatzigzagline{\pgfpointanchor{frame}{south east}}{\pgfpointanchor{frame}{south west}}%
      \pgfpathclose%
      \pgfsetfillcolor{tcbcolback}%
      \pgfsetfillopacity{1}%
      \pgfsetstrokecolor{tcbcolframe}%
      \pgfsetstrokeopacity{1}%
      \pgfsetlinewidth{0.9pt}%
      \pgfusepath{fill,stroke}%
      \end{pgfscope}%
    },
    underlay middle={%
      \begin{pgfscope}%
      \pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
      \pgfpathmoveto{\pgfpointanchor{frame}{north west}}%
      \chatzigzagline{\pgfpointanchor{frame}{north west}}{\pgfpointanchor{frame}{north east}}%
      \pgfpathlineto{\pgfpointanchor{frame}{south east}}%
      \chatzigzagline{\pgfpointanchor{frame}{south east}}{\pgfpointanchor{frame}{south west}}%
      \pgfpathclose%
      \pgfsetfillcolor{tcbcolback}%
      \pgfsetfillopacity{1}%
      \pgfsetstrokecolor{tcbcolframe}%
      \pgfsetstrokeopacity{1}%
      \pgfsetlinewidth{0.9pt}%
      \pgfusepath{fill,stroke}%
      \end{pgfscope}%
    },
    underlay last={%
      \begin{pgfscope}%
      \pgfsetcornersarced{\pgfqpoint{0pt}{0pt}}%
      \pgfpathmoveto{\pgfpointanchor{frame}{north west}}%
      \chatzigzagline{\pgfpointanchor{frame}{north west}}{\pgfpointanchor{frame}{north east}}%
      \pgfsetcornersarced{\pgfqpoint{2pt}{2pt}}%
      \pgfpathlineto{\pgfpointanchor{frame}{south east}}%
      \pgfpathlineto{\pgfpointanchor{frame}{south west}}%
      \pgfpathclose%
      \pgfsetfillcolor{tcbcolback}%
      \pgfsetfillopacity{1}%
      \pgfsetstrokecolor{tcbcolframe}%
      \pgfsetstrokeopacity{1}%
      \pgfsetlinewidth{0.9pt}%
      \pgfusepath{fill,stroke}%
      \end{pgfscope}%
    },
    before upper={%
      \setlength{\parskip}{0.5\baselineskip}%
    },
  },
  numbered/.style={
    left=8mm,
    before upper={%
      \setlength{\parskip}{0.5\baselineskip}%
      \setcounter{paranum}{0}%
      \def\paranumlabel{\refstepcounter{paranum}\llap{\textcolor{canvas!40!black}{\texttt{\textpilcrow\theparanum}}\hspace{2mm}}}%
      \everypar{\paranumlabel}%
      \let\oldpar\par%
      \def\par{\ifhmode\vadjust{\vskip0.5\baselineskip}\fi\oldpar}%
    },
  },
  linenumbered/.style={
    left=6mm,
    before upper={%
      \setlength{\parskip}{0.5\baselineskip}%
      \internallinenumbers%
      \resetlinenumber%
      \modulolinenumbers[5]%
      \linenumbersep=2mm%
      \renewcommand{\thelinenumber}{\rmfamily\scriptsize\textcolor{canvas!30!black}{\arabic{linenumber}}}
      % \renewcommand\thelinenumber{\roman{linenumber}}
      % \def\makeLineNumber{\llap{\rmfamily\scriptsize\textcolor{canvas!50!black}{\LineNumber}\hspace{2mm}}}%
    },
  },
}

\newtcolorbox[auto counter]{prompt}[1][]{%
  chatbox,
  title={\lsstyle\uppercase{prompt~\thetcbcounter}},
  coltitle=persimmon,
  boxed title style={
    colback=canvas,
    colframe=persimmon,
  },
  colframe=persimmon,
  colback=goldenrod!70!white,
  attach boxed title to top right={yshift=-3mm,xshift=-4mm},
  #1
}

\newtcolorbox[auto counter,use counter from=prompt]{llm}[1][]{%
  chatbox,
  title={\lsstyle\uppercase{llm response~\thetcbcounter}},
  coltitle=persimmon,
  boxed title style={
    colback=canvas,
    colframe=persimmon,
  },
  colframe=canvas!80!black,
  colback=canvas!70!white,
  #1
}

\def\faint#1{{\color{canvas!60!black}#1}}

\newlength{\llmfillerskip}
\setlength{\llmfillerskip}{-0.5\baselineskip} 

\newcommand{\llmfiller}{%
\par
{\hfill\sffamily\faint{[...]}\hfill}
\par
% \vspace{1em}
% {\centering \faint{...}}\null
  % \let\oldep\everypar
  % \ifhmode\vadjust{\vskip0.5\baselineskip}\fi\par\vspace{\llmfillerskip}%
  % \begin{center}{\sffamily [...]}\end{center}%
  % \vspace{1\llmfillerskip}%
  % \everypar{\paranumlabel}\par%
  % \let\everypar\oldep
}

\newcommand{\parref}[1]{\textpilcrow\ref{#1}}

%% Custom macros
\newcommand\WM[1]{\textsf{\color{orange} WM: #1}}
\newcommand\JP[1]{\textsf{\color{teal} JP: #1}}
\newcommand\MH[1]{\textsf{\color{purple} MH: #1}}
\newcommand\TL[1]{\textsf{\color{blue} TL: #1}}
\newcommand\TODO[1]{\textsf{\color{red}\bfseries TODO: #1}}
\newcommand\SR[1]{\textsf{\color{cyan} SR: #1}}
\newcommand\LLM[1]{{\ttfamily\color{black!60}#1}}

% Define commands for colored symbols
\newcommand{\greencheck}{{\color{mygreen}\checkmark}}
\newcommand{\redx}{{\color{myred}$\times$}}

\def\TASKNAME{\text{RELIC}}
\let\RELIC\TASKNAME

\newcommand\NC{\mathsf{NC}}
\newcommand\AC{\mathsf{AC}}
\newcommand\TC{\mathsf{TC}}

\renewcommand\P{\mathsf{P}}

\def\Nterm{\ensuremath{n_\text{term}}}
\def\Nnonterm{\ensuremath{n_\text{nonterm}}}
\def\Nlex{\ensuremath{n_\text{lex}}}
\def\Nnonlex{\ensuremath{n_\text{nonlex}}}
\def\tok#1{\texttt{#1}}

